AnswerSumm: A Manually-Curated Dataset and Pipeline for Answer Summarization

Community Question Answering (CQA) fora such as Stack Overflow and Yahoo! Answers contain a rich resource of answers to a wide range of community-based questions. Each question thread can receive a large number of answers with different perspectives. One goal of answer summarization is to produce a summary that reflects the range of answer perspectives. A major obstacle for this task is the absence of a dataset to provide supervision for producing such summaries. Recent works propose heuristics to create such data, but these are often noisy and do not cover all answer perspectives present. This work introduces a novel dataset of 4,631 CQA threads for answer summarization curated by professional linguists. Our pipeline gathers annotations for all subtasks of answer summarization, including relevant answer sentence selection, grouping these sentences based on perspectives, summarizing each perspective, and producing an overall summary. We analyze and benchmark state-of-the-art models on these subtasks and introduce a novel unsupervised approach for multi-perspective data augmentation that boosts summarization performance according to automatic evaluation. Finally, we propose reinforcement learning rewards to improve factual consistency and answer coverage and analyze areas for improvement.

==> prev/misc_save.tex <==
% SECTION: old text re data part
% % \par
% We found that a BART model trained on CQASumm was almost entirely extractive, likely due to how the dataset was filtered. We found fewer hallucinations when the model was trained on the dataset filtered by entailment and fewer with the model filtered according to named entities. For these models, the types of hallucinations found were sometimes plausible answers, even though the answer was not stated directly in the source documents. We show a comparison of our data and some characteristics to \ref{tab:statistics}. 
% \subsection{Alternative Pipeline}
% We explore an alternative dataset creation pipeline centered on sub-aspects of summarization as detailed in \citet{jung-etal-2019-earlier}. This paper introduces quantitative notions of position, importance and diversity in existing summarization datasets. Importance is defined by correlation of dimension-reduced sentence embeddings. Diversity is defined by coverage in a convex hull. Specifically, we use their N-nearest formulation of importance, which calculates an averaged Pearson correlation between one sentence and the rest for the source sentence vector representations and picks the summaries with the highest averaged correlations. For diversity we make use of their ConvexFall algorithm which prunes redundant sentences from those chosen by the convex-hull search. We first extract the 10 most important sentences and then use the ConvexFall algorithm to prune sentences, keeping a max of 4 sentences (as this was the average number of sentences in our original pipeline). We find fairly similar trends for the two datasets in terms of statistics and baselines (this pipeline vs our original pipeline); length of 69 vs 75, novel unigrams 0.37 vs 0.34, repeated unigrams (0.22 vs 0.20). The BART baseline trained and validated on this dataset has a ROUGE-1 of 0.344 vs 0.325 for the model trained and validated on our data. However, running the model on this pipeline data and using the validation data created in our pipeline returns very similar ROUGE scores. 




% SECTION: misc old tables
% \newcommand{\DatasetComparison}{
%  \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{c c c c c c } \Xhline{2\arrayrulewidth}
%              \textbf{Dataset} & \textbf{Novel unigrams} &  \textbf{Repeated unigrams}  &  \textbf{Oracle Extractive}  &  \textbf{Length}  &  \\ \Xhline{\arrayrulewidth}
%              Our Dataset & 0.24 & 0.20 &  40.22/10.93/35.52 & 75  \\ 
%             XSUM & 0.33 & 0.05 & 29.79/8.81/22.65 & 24 \\
%              CNN-DailyMail & 16.75 & 0.10 & 50.38/28.55/46.58 & 45.70 \\
%             \Xhline{2\arrayrulewidth}
% \end{tabular}
% \caption{Comparison of statistics between our proposed dataset pipeline and the standard XSum \cite{narayan-etal-2018-dont} and CNN-DailyMail \cite{nallapati-etal-2016-abstractive} summarization datasets. }
% \label{tab:statistics}
% \end{table*}
% }

% \newcommand{\BaselineResults}{
% \begin{table}[t!]
% \small
% \resizebox{\columnwidth}{!}{\begin{tabular}{|l|ccc|}
% \hline
%     \textbf{Method}   & \textbf{ROUGE-1}    & \textbf{ROUGE-2}    & \textbf{ROUGE-L}    \\ \hline \hline
% LexRank	&	26.65	&	4.84	&	23.32	\\
% TextRank	&	28.61	&	4.98	&	24.75	\\
% BertSum &	29.82	&	5.51	&	25.28	\\
% \hline
% \end{tabular}}
% \caption{ROUGE scores for baseline extractive models.}
% \label{tab:baseline_results}
% \end{table}
% }

